Online Subset Selection using $\alpha$-Core with no Augmented Regret

We revisit the classic problem of optimal subset selection in the online learning set-up. Assume that the set $[N]$ consists of $N$ distinct elements. On the $t$th round, an adversary chooses a monotone reward function $f_t: 2^{[N]} \to \mathbb{R}_+$ that assigns a non-negative reward to each subset of $[N].$ An online policy selects (perhaps randomly) a subset $S_t \subseteq [N]$ consisting of $k$ elements before the reward function $f_t$ for the $t$th round is revealed to the learner. As a consequence of its choice, the policy receives a reward of $f_t(S_t)$ on the $t$th round. Our goal is to design an online sequential subset selection policy to maximize the expected cumulative reward accumulated over a time horizon. In this connection, we propose an online learning policy called SCore (Subset Selection with Core) that solves the problem for a large class of reward functions. The proposed SCore policy is based on a new polyhedral characterization of the reward functions called $\alpha$-Core - a generalization of Core from the cooperative game theory literature. We establish a learning guarantee for the SCore policy in terms of a new performance metric called $\alpha$-augmented regret. In this new metric, the performance of the online policy is compared with an unrestricted offline benchmark that can select all $N$ elements at every round. We show that a large class of reward functions, including submodular, can be efficiently optimized with the SCore policy. We also extend the proposed policy to the optimistic learning set-up where the learner has access to additional untrusted hints regarding the reward functions. Finally, we conclude the paper with a list of open problems.

==> local_weak_submodularity.tex <==
\section{Local Weak Submodularity}
%
\label{sec:local-weak-submodularity}
Let $f$ be a monotone set function, i.e., $f(S)\le f(T)$, whenever $S\subseteq T$. Furthermore, assume that $f(\emptyset) = 0$. We define a new property of such a set function as below:
\begin{definition}[\textbf{Local Weak Submodularity}]
    \label{def:local-weak-submodularity}
    A monotone set function $f$ is said to be \emph{locally weak $\beta-$submodular} for some $\beta\ge 0$, if the following is satisfied for any set $S\subset [n]$ and for any $x,y\notin S$:
    \begin{align}
        \label{eq:local-weak-submodularity}
        f(S\cup\{x\}) - f(S) & \ge \beta (f(S\cup \{x,y\}) - f(S\cup \{y\})).
    \end{align}
\end{definition}
The following is a straightforward consequence of Definition~\ref{def:local-weak-submodularity}:
    \begin{proposition}
    \label{prop:weak-local-submodularity-submodularity-equivalence}
    A locally weak $\beta$-submodular function is submodular if and only if $\beta\ge 1$.
    \end{proposition}
    \begin{proof}
    \colr{\textbf{SM:} The proof is simple. Need to write a few lines about it.}
    \end{proof}
    In the rest of the treatment, we will be interested in the case $\beta<1$. 
    We now recall the definition of submodularity ratio from~\cite{das2018approximate}:
    \begin{definition}[{\bf Submodularity Ratio}]
        A monotone function $f$ is said to have a submodularity ratio $\gamma$ if, for any two sets $S,T\subseteq[n]$,
        \begin{align}
            \label{eq:submodualrity-ratio}
            \sum_{x\in T\setminus S} (f(S\cup \{x\}) - f(S)) & \ge \gamma (f(S\cup T)-f(S)).
        \end{align}
    \end{definition}
    It turns out that the notion of locally weak $\beta-$submoduarity is intrinsically connected to submodularity ratio. To see this, our first observation is that $\beta\ge 1\Longleftrightarrow \gamma\ge 1$. Indeed, by Proposition~\ref{prop:weak-local-submodularity-submodularity-equivalence}, the condition $\beta\ge 1$ is equivalent to submodularity, which, due to Proposition 3 of~\cite{das2018approximate}, is equivalent to $\gamma\ge 1$. It remains to investigate the connection between the conditions $\beta<1$ and $\gamma<1$. In this regard, we first prove the following property of a locally weak $\beta$-submodular function:
    %
    \begin{proposition}
        For any monotone set function with submodularity ratio $\gamma<1$, the function is locally weak $\beta$-submodular, with $\beta\le \gamma^{\frac{1}{n-1}}$.
    \end{proposition}
    \begin{proof}
        Let us consider any two sets $S,T\subseteq[n]$, such that $S\ne T$. Let $T=S\cup \{x_1,\cdots, x_l\}$. Since $f$ is locally weak $\beta$-submodular, for any $1\le k\le l$, 
        \begin{align}
            f(S\cup \{x_k\})-f(S) & \ge \beta\big(f(S\cup \{x_k,x_{k-1}\})-f(S\cup\{x_{k-1}\})\big)\nonumber\\
            \ & \ge \cdots \ge \beta^{k-1}\big(f(S\cup \{x_k,x_{k-1},\cdots, x_1\})-f(S\cup\{x_{k-1},\cdots, x_1\})\big).
        \end{align}
        Let $S_i=\{x_1,\cdots, x_i\}$, for $1\le i\le k$, and $S_0=\emptyset$. Then, we have, for any $1\le k\le l$,
        \begin{align}
            f(S\cup \{x_k\})-f(S) & \ge \beta^{k-1}\big(f(S\cup S_k)-f(S\cup S_{k-1})\big).
        \end{align}
        Consequently, we obtain,
        \begin{align}
            \ & \sum_{k=1}^l \big(f(S\cup \{x_k\})-f(S)\big) \ge \sum_{k=1}^l \beta^{k-1} \big(f(S\cup S_k)-f(S\cup S_{k-1})\big)\ge \beta^{l-1}\big(f(S\cup T)-f(S)\big).
        \end{align}
        Therefore, 
        \begin{align}
            \gamma = \min_{S,T}\frac{\sum_{x\in T\setminus S}\big(f(S\cup \{x_k\})-f(S)\big)}{f(S\cup T)-f(S)} & \ge \min_{1\le l\le n}\beta^{l-1}=\beta^{n-1}.
        \end{align}
    \end{proof}
    Proposition~\ref{prop:weak-local-submodularity-submodularity-equivalence} allows one to work with the local weak submodularity of a set function if it has a submodualrity ratio $\gamma\le 1$. If the function $f$ satisfies $A\le f(S)\le B$ for any $S\subseteq[n]$, then we can obtain a further connection between $\beta$ and $\gamma$ as below:
    \begin{corollary}
        Let $A\le f(S) \le B$ for all $S\subseteq [n]$ and $\omega = B/A$. Then, for any monotone set function $f$ the following is satisfied:
        \begin{align}
            \label{eq:beta-lower-bound}
            \beta & \ge \frac{\gamma}{1+\omega(1-\gamma)}.
        \end{align}
    \end{corollary}
    \begin{proof}
        Let $S, x,y\notin S$ are such that,
        \begin{align}
            \beta = \frac{f(S\cup \{x\})-f(S)}{f(S\cup \{x,y\})-f(S\cup \{y\})}.
        \end{align}
        Let us denote $a = f(S\cup \{x\})-f(S)$ and $b = f(S\cup \{y\})-f(S)$. Then note that
        \begin{align}
            f(S\cup \{x,y\}) - f(S) & = a/\beta + b.
        \end{align}
        Also, we have,
        \begin{align}
            \ & \frac{f(S\cup \{y\})-f(S)}{f(S\cup \{x,y\})-f(S\cup \{x\})} \ge \beta\nonumber\\
            \ & \Longleftrightarrow \frac{b}{\frac{a}{\beta} + b - a} \ge \beta\nonumber\\
            \ & \Longleftrightarrow b \ge a\quad (\because \beta<1).
        \end{align}
        Then, we have, 
        \begin{align}
            \frac{a+b}{\frac{a}{\beta}+b} \ge \gamma & \Longleftrightarrow \beta\left(\frac{1 + c}{1+\beta c}\right) \ge \gamma\quad (c = b/a).
        \end{align}
        Since the function $\frac{1+c}{1+\beta c}$ is increasing in $c$ as $\beta<1$, and $c\le B/A:=\omega$, we obtain the following:
        \begin{align}
            \beta\left(\frac{1 + \omega}{1+\beta \omega}\right) \ge \gamma\implies \beta \ge \frac{\gamma}{1+\omega(1-\gamma)}.
        \end{align}
    \end{proof}
    To see how this connection can be leveraged, we now turn our attention to a novel solution concept in coalition games with transferable utility (TU). In the following, we will denote $N=[n]$. 
    \begin{definition}[\textbf{$\alpha \text{ -}$core of order $k$}]
        Let $(N,f)$ be a TU cost game. For any $\alpha>0$, the \emph{$\alpha$-core} of order $1\le k\le n$ is defined as the set $\core{\alpha}{k}{f}$ containing all vectors $\bm{x}\in \real^n$ satisfying the following:
        \begin{align}
            \sum_{i\in S}x_i & \le \alpha f(S),\ \forall S\subseteq N: |S|=k,\nonumber\\
            \sum_{i\in N}x_i & =  f(N).
        \end{align}
    \end{definition}
    Using this definition, we now prove the following main result:
    \begin{theorem}
        For a TU cost game $(N,f)$ with locally weak $\beta$-submodular cost function $f$, $\core{\alpha}{k}{f}$ is nonempty whenever $\alpha\ge \beta^{-(n-k)}$.
    \end{theorem}
    \begin{proof}
        We use the technique of~\cite{maschler2020game} for constructing a vector and subsequently obtaining a condition on $\alpha$ which ensures that it is an element of $\core{\alpha}{k}{f}$. 
        
        Let us construct the following vector $\bm{x}\in \real^n$:
        \begin{align}
        \begin{array}{ll}
             x_1 & = f(\{1\}),\\
             x_2 & = f(\{1,2\}) - f(\{1\}),\\
            \ & \vdots\\
             x_n & = f(\{1,2,\cdots, n\}) - f(\{1,2,\cdots, n-1\}).
        \end{array}
        \end{align}
        Then it immediately follows that $\sum_{i\in N}x_i = f(N)$. Now, consider any set $S=\{i_1,i_2,\cdots, i_k\}$ of size $k$ and ordering $1\le i_1<i_2<\cdots <i_k\le n$. Then, we have,
        \begin{align}
            \sum_{j\in S}x_j & = \sum_{l=1}^k x_{i_l}= \sum_{l=1}^k \big(f(\{1,2,\cdots, i_l\}) - f(\{1,2,\cdots, i_{l}-1\})\big).
        \end{align}
        Now, using similar arguments as in the proof of Proposition~\ref{prop:weak-local-submodularity-submodularity-equivalence}, we obtain
        \begin{align}
            f(\{1,2,\cdots, i_l\}) - f(\{1,2,\cdots, i_{l}-1\}) & \le \beta^{-(i_l-l)}\big(f(\{i_1,i_2,\cdots, i_l\}) - f(\{i_1,i_2,\cdots, i_{l-1}\})\big).
        \end{align}
        Therefore,
        \begin{align}
            \sum_{j\in S}x_j & = \sum_{l=1}^k x_{i_l}\nonumber\\
            \ & \le \sum_{l=1}^k \beta^{-(i_l-l)}\big(f(\{i_1,i_2,\cdots, i_l\}) - f(\{i_1,i_2,\cdots, i_{l-1}\})\big)\nonumber\\
            \ & \stackrel{(a)}{\le} \beta^{-(n-k)}\sum_{l=1}^k\big(f(\{i_1,i_2,\cdots, i_l\}) - f(\{i_1,i_2,\cdots, i_{l-1}\})\big) = \beta^{-(n-k)}f(S),
        \end{align}
        where step $(a)$ follows from the observation that $i_l\le n-k+l$ as $1\le i_1<i_2<\cdots <i_k\le n$ and the monotonicity of $f$.
    \end{proof}
    

==> partialinfo.tex <==
\section{Online Subset Selection under Semi-Bandit Feedback}\label{partialinfo}
%\subsection{Semi-Bandit Version}
In this section, we extend the online subset selection policy for linear rewards, given in Algorithm \ref{linear-reward-algo}, to the semi-bandit feedback model. Recall that in the semi-bandit model, the learner receives the components of the reward vector, $g_t(i)$, only for the elements $i\in S_t$ in the subset selected by the learner on round $t$. As before, the learner's objective is to attain a sublinear expected regret defined in Theorem~\ref{lin-reward}. Here, the expectation is taken over all internal randomizations of the algorithm.

 In Algorithm \ref{semibandit-linear}, we propose a simple extension of Algorithm \ref{linear-reward-algo}, where we use the \emph{inverse propensity scoring} (step \ref{ips-step} in Algorithm \ref{semibandit-linear}) to estimate the unobserved coordinates. Note that no explicit exploration term is included in Algorithm \ref{semibandit-linear}. In the following, we analyze the static regret bound achieved by this policy. 

%We build on the works on \cite{kale2010non} in the context of bandit slate problem and present the algorithm in Algorithm~\ref{semibandit-linear}. It is to be noted that although \cite{kale2010non} term their problem as a bandit problem, by the definition of this work, it is actually in a semi-bandit setting.


\begin{algorithm}
\caption{Online Subset Selection Policy with \textsc{Linear-rewards} (Semi-bandit feedback)}
\label{semibandit-linear}
\begin{algorithmic}[1]
%\REQUIRE Define $\bm p_1 = \frac{k}{N}\bm 1, \eta >0$.
\REQUIRE Sequence of linear reward functions $\{f_t\}_{t \geq 1}$ with coefficients $\{\bm{g}_t\}_{t\geq 1}, \eta >0$.
\STATE $\bm{p} \gets (\frac{k}{N}, \frac{k}{N}, \ldots, \frac{k}{N}).$
\FOR {every round $t$:}
% \STATE Set $\bm p'_t = (1-\gamma)\bm p_t + \gamma \bm p_1.$
\STATE Sample a $k$-set according to the inclusion probability vector $\bm{p}$ using Madow's algorithm ~\ref{uneq} 
%with the inclusion probability vector $\bm p_t$ computed above.

%\textsc{Semi-bandit setting (line 5 and 6)}
\STATE Receive the reward components of the coefficient vector $\bm{g}_t$ on the selected subset $\{g_{t,i}, \forall i\in S_t\}$.
\STATE Set $\hat{g}_{t, i}\gets \frac{g_{t,i}}{ p_{t,i}}$ for $i\in S_t$ and $0$ otherwise. \textcolor{blue}{// Inverse propensity scores} \label{ips-step}
\STATE Feed the estimated vector $\bm{\hat{g}}_t$ and update the inclusion probability vector $\bm{p}$ according to the \textsc{FTRL}($\eta$) update \eqref{ftrl-opt}.
%\textsc{Bandit setting (line 7 and 8)}
%\STATE Observe $\langle\bm g_t, \chi_{S_t}\rangle$.
%\STATE Set $\hat{\bm g}_t=M^\dagger\chi_{S_t}\chi_{S_t}^\top \bm g_t $ where $M = \mathbb{E}\left[\chi_{S_t}\chi_{S_t}^\top\right]$ and $X^\dagger$ is Moore-Penrose inverse of $X$.
%
%
%\STATE Feed the vector $\hat{\bm g}_t$ as the reward vector for round $t$ to the \textsc{FTRL}($\eta$) policy 
\ENDFOR
\end{algorithmic}
\end{algorithm}

\paragraph{Analysis:}

Note that, by definition, the estimated components of the reward vectors are unbiased as
\begin{align}
  \mathbb{E}[\hat{g}_{t, i}]=\sum_{S: i \in S}q_t(S)\frac{g_{t,i}}{ p_{t,i}}=   \frac{g_{t, i}}{p_{t,i}}\sum_{S: i \in S}q_t(S)=g_{t, i},  
\end{align}
where $q_t(S)$ is the (conditional) probability of choosing the $k$-set $S$. The last equality holds as $p_{t,i} = \sum_{i \in S} q(S)$. Thus we have that
$\mathbb{E}[\langle \hat{\bm g_t}, \bm p\rangle]=\langle \bm g_t, \bm p\rangle$ for any vector $\bm p$.

 Now recall the following standard static regret bound for the \textsc{FTRL}($\eta$) policy from \citet[Theorem 5.2]{hazan2019introduction}. For a bounded, convex and closed set $\Omega$ and a strongly convex regularization function $R: \Omega \to \mathbb{R},$ consider the standard \textsc{FTRL} updates, \emph{i.e.},
 \begin{eqnarray}\label{ftrl-updates}
  \bm{x}_{t+1} = \arg\max_{\bm{x} \in \Omega}\left[ \left(\sum_{s=1}^t \nabla_s^\top\right) \bm{x} - \frac{1}{\eta}R(x), \right]   
 \end{eqnarray} 
 where $\nabla_s= \nabla f_t(\bm{x}_s), \forall s$. Taking $\Omega \equiv \Delta^N_k$ to be the capped-simplex defined by \eqref{necsuf1} and \eqref{necsuf2} and $R(\bm{x}) \equiv \sum_{i=1}^N x_i \ln x_i$ to be the entropic regularizer, the regret of the \textsc{FTRL}($\eta$) policy can be upper-bounded as follows:
  \begin{eqnarray}\label{reg-bd-main}
  \textrm{Regret}^{\textrm{FTRL}}_T \leq 2 \eta \sum_{t=1}^T || \nabla_t||_{*,t}^2 + \frac{R(\bm{u})-R(\bm{x}_1)}{\eta},
  \end{eqnarray}

 where the quantity $||\nabla_t||_{*,t}^2$ denotes the square of the dual norm of the vector induced by the Hessian of the regularizer evaluated at some point $\bm{x}_{t+1/2}$ lying in the line segment connecting the points $\bm{x}_t$ and $\bm{x}_{t+1}$. Hence, for the \textsc{Linear-reward} problem with the sequence of reward vectors $\hat{\bm g}_1, \dots, \hat{\bm g}_T$, we have:
\begin{align}
    \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle \hat{\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle \hat{\bm{g}}_t, \bm{p}_t \rangle \leq 2 \eta \sum_{t=1}^T || \nabla_t||_{*,t}^2 + \frac{R(\bm{u})-R(\bm{x}_1)}{\eta},
\end{align}
The following diagonal matrix gives the Hessian of the entropic regularizer: 
 \begin{eqnarray*}
 \nabla^2 R(\bm{p}_{t+1/2}) = \textrm{diag}([p_1^{-1}, p_2^{-1}, \ldots, p_N^{-1}])\implies || \nabla_t||_{*,t}^2 =\langle \bm p_t, \hat{\bm g}^2_t\rangle,
 \end{eqnarray*}
In the above, the vector $\hat{\bm g}_t^2$ is obtained by squaring each component of the vector $\hat{\bm g}_t.$ To bound the second term in \eqref{reg-bd-main}, define a probability distribution $\tilde{\bm{p}} = \bm{p}/k.$ We have 
 \begin{eqnarray*}
 0 \geq R(\bm{p})  = \sum_i p_i \ln p_i = - k \sum_i \tilde{p}_i \ln \frac{1}{p_i}\stackrel{\textrm{(Jensen's inequality)}}{\geq} -k \ln \sum_i \frac{\tilde{p}_i}{p_i} = -k \ln \frac{N}{k}.   	
 \end{eqnarray*}
Hence, for this problem, the general regret bound in \eqref{reg-bd-main} simplifies to the following:
\begin{eqnarray*}
 \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle \hat{\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle \hat{\bm{g}}_t, \bm{p}_t \rangle \leq \frac{k}{\eta} \ln \frac{N}{k}+ 2\eta \sum_{t=1}^T \langle \bm p_t, \hat{\bm g}^2_t\rangle. 
\end{eqnarray*}
Taking expectations of both sides with respect to the random choice of the policy and using Jensen's inequality, we have
\begin{align}\label{r1}
   \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}_t \rangle \leq \frac{k}{\eta} \ln \frac{N}{k}+ 2\eta \sum_{t=1}^T \mathbb{E}\left[\langle \bm p_t, \hat{\bm g}^2_t\rangle\right],  
\end{align}
where we have used the fact that the estimated rewards are unbiased. 
Now, notice that
\begin{align}\label{r2}
    \mathbb{E}\left[ \langle \bm p_t, \hat{\bm g}^2_t\rangle\right] &= \sum_{S \subseteq [N]}q_t(S) \sum_{i\in S}p_{t,i}\frac{g_{t,i}^2}{p_{t,i}^2}=\sum_{i=1}^N\frac{g_{t,i}^2}{p_{t,i}}\sum_{S \ni i}q_t(S)\stackrel{(a)}{=}\sum_{i=1}^Ng_{t,i}^2\leq G^2,
\end{align}
where (a) holds because $\sum_{S\ni i}q(S)=p_{t,i}$, and  by definition $||\bm g_t||_2^2\leq G^2$. 
% Furthermore,
% \begin{align}\label{r3}
%     \langle\bm g_t, \bm p_t\rangle - \langle\bm g_t, \bm p_t'\rangle = \gamma\langle\bm g_t, \bm p_t-\bm p_1\rangle\leq \gamma||\bm g_t||_\infty||\bm p_t-\bm p_1||_1\leq\gamma(||\bm p_t||_1+||\bm p_t||_1)= 2\gamma k
% \end{align}
Combining results from \eqref{r1} and \eqref{r2}, we have:
\begin{align}\label{linear-reward-semi}
  \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}_t \rangle \leq \frac{k}{\eta} \ln \frac{N}{k}+ 2\eta G^2T 
%   \frac{NT}{1-\gamma}+2\gamma kT. 
\end{align}

Setting $\eta=\sqrt{\dfrac{k \ln (N/k)}{2G^2T}}$, we get the following static regret bound
\begin{align} \label{semi-bandit-regret}
   \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}_t \rangle \leq 2G\sqrt{2kT\ln \frac{N}{k}},
\end{align}
where $G$ is a uniform upper bound to the $\ell_2$ norms of the reward vectors $\{\bm{g}_t, t \geq 1\}.$

%For $(\alpha, k)$-admissible reward functions, the learner can only observe those coordinates of $g_t\in\core{\alpha, k}{f}$ which are chosen by her earlier in the round.
\subsection*{Regret bound for learning non-linear reward functions under semi-bandit feedback}

Observe that in the complete information setting, The \onscore policy, described in Algorithm \ref{monotone-reward-algo}, uses only the reward vector $\bm{g}_t $ and \textit{not} the entire set function $f_t$. We use a feedback model similar to~\cite{takemori20a}, where marginal gains for the items chosen in set $S_t$ are observed when the reward functions are submodular. Consequently, we define the subset selection problem for $\alpha$-admissible functions in the semi-bandit setting as follows: at any round $t$, the learner plays a $k$-set $S_t$, and the adversary reveals the selected reward components $\{g_{t,i}, i\in S_t\}$ for some $\bm g_t\in\core{\alpha}{f_t}$. Then, we use Algorithm~\ref{semibandit-linear} to construct an unbiased estimator $\hat{\bm g}_t$ and subsequently update the weights. Finally, the same augmented regret bound given in \eqref{regret-guarantee1} follows immediately in the semi-bandit setting using the inequalities \eqref{est1} and \eqref{est2} and the semi-bandit regret bound in \eqref{linear-reward-semi}. From Proposition \ref{core-bd}, for $\alpha$-admissible reward functions taking values in $[0, M],$ we can take $G \equiv \alpha M\sqrt{2}$. It is easy to see that the space and time complexity of the semi-bandit version is of the same order as in the complete information setting.

%\cmt{SS: Rationale for hiding $g_t$ instead of $f_t$: In the partial information setting, the core idea is to construct an unbiased estimator of loss/reward vector, i.e., $\mathbb{E}[\hat{l}_t]=l_t$. Note that Algorithm \ref{monotone-reward-algo} uses the reward vector $g_t$ for updating the weights. Consider two set functions $f_1$ and $f_2$ that yield the same $g_t$. So, constructing a consistent unbiased estimator is not feasible, i.e., $\mathbb{E}[\hat{f}]$ can be either $f_1$ or $f_2$. So, in the general subset selection problem, we define the semi-bandit version as follows: at any round $t$, the learner plays a $k$-set $S_t$, the adversary reveals $g_{t,i}, i\in S_t$ where $\bm g_t\in\core{\alpha, k}{f_t}$. A similar argument has been put forward by~\cite[Section 4]{takemori2020submodular} and \cite[Section 2]{uchiya2010algorithms}. Then, the result follows immediately using the arguments from \eqref{est1} and \eqref{est2} and the bound for \eqref{linear-reward-semi}. }


%\subsection{Bandit Version}
%
%In the bandit setting of the \textsc{Linear-reward} of the problem, at the end of each round $t$, the learner receives only $\langle \bm g_t, \chi_{S_t}\rangle$ where $\chi_{S}$ is the characteristic vector of set $S$ defined as $\chi_S(i)=\bm 1(i\in S)$. The learner aims to attain sublinear expected regret defined in Theorem~\ref{lin-reward}. Following the study by ~\cite{bubeck2012towards} on bandit online linear optimization, we present the algorithm in Algorithm~\ref{semibandit-linear}. 
%
%\textbf{Analysis:}
%Note that,
%\begin{align}
%    \mathbb{E}[\hat{\bm g_t}] = M^\dagger\mathbb{E}\left[\chi_{S_t}\chi_{S_t}^\top\right]\bm g_t = M^\dagger M\bm g_t
%\end{align}
%If $M$ is invertible, then, $\hat{\bm g_t}$ is an unbiased estimator of $\bm g_t$. Following an analysis similar to that of the semi-bandit version, we get the following regret bound,
%
%\begin{align}\label{linear-reward-bandit}
%   \max_{\bm{p}^* \in \Delta^N_k} \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}^* \rangle - \sum_{t \leq T} \langle {\bm{g}}_t, \bm{p}'_t \rangle \leq \frac{k}{\eta} \ln \frac{N}{k} + 2\eta\sum_{t=1}^T\mathbb{E}\left[\langle \bm p_t, \hat{\bm g_t}^2\rangle\right]. 
%\end{align}
%
%\textbf{Computing $M$:}
%\begin{align}
%    M = \mathbb{E}\left[\chi_{S}\chi_{S}^\top\right]=\sum_{S}q(S)\chi_{S}\chi_{S}^\top\implies M_{ij} = \sum_{i,j\in S}q(S)
%\end{align}
%So, $M_{ij}$ is the second-order marginal inclusion probabilities of experts $i$ and $j$. This joint inclusion probability matrix can be computed exactly in $O(N^2)$ time~\citep{tille2006sampling}.
% \begin{algorithm}
% \caption{Partial Information Setting Algorithm for Subset Selection with \textsc{Linear-reward}}
% \label{bandit-linear}
% \begin{algorithmic}[1]
% \REQUIRE Define $\bm p_1 = \frac{k}{N}\bm 1, \eta, \gamma$.
% \FOR {every round $t$:}
% \STATE Obtain $\bm p_t$ from \textsc{FTRL}($\eta$) policy.
% \STATE Set $\bm p'_t = (1-\gamma)\bm p_t + \gamma \bm p_1.$
% \STATE Sample a $k$-set using Algorithm~\ref{uneq} with $\bm p'_t$ and .

% \textsc{Semi-bandit setting (line 5 and 6)}
% \STATE Observe $g_{t,i}, \forall i\in S_t$.
% \STATE Set $\hat{g}_{t, i}=\frac{g_{t,i}}{ p'_{t,i}}$ for $i\in S_t$ and 0 otherwise.

% \textsc{Bandit setting (line 7 and 8)}
% \STATE Observe $\langle\bm g_t, \chi_{S_t}\rangle$.
% \STATE Set $\bm \hat{g}_t=M^\dagger\chi_{S_t}\chi_{S_t}^\top \bm g_t $ where $M = \mathbb{E}\left[\chi_{S_t}\chi_{S_t}^\top\right]$ and $X^\dagger$ is Moore-Penrose inverse of $X$.


% \STATE Feed the vector $\hat{\bm g}_t$ as the reward vector for round $t$ to the \textsc{FTRL}($\eta$) policy 
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}


==> related.tex <==
\section{Related Work} \label{related work}
In this section, we briefly describe related works on online learning in general and online subset selection in particular.
\citet{streeter2007online} designed the first online $k$-set selection algorithm for maximizing submodular functions, achieving a sublinear $(1-1/e)$-regret. Their algorithm essentially runs $k$ experts algorithms with the marginal gains as the rewards \cmt{explain}. 

